A loss discounting framework for model averaging and selection in time series models

We introduce a Loss Discounting Framework for model and forecast combination which generalises and combines Bayesian model synthesis and generalized Bayes methodologies. We use a loss function to score the performance of different models and introduce a multilevel discounting scheme which allows a flexible specification of the dynamics of the model weights. This novel and simple model combination approach can be easily applied to large scale model averaging/selection, can handle unusual features such as sudden regime changes, and can be tailored to different forecasting problems. We compare our method to both established methodologies and state of the art methods for a number of macroeconomic forecasting examples. We find that the proposed method offers an attractive, computationally efficient alternative to the benchmark methodologies and often outperforms more complex techniques.

==> tables/table_ecb.tex <==
\begin{tabular}{c|c|c||c|c|c}
\textbf{Model}  & $\mbox{MLS}$    & $\sum \log(p)$      & \textbf{Model} & $\mbox{MLS}$ & $\sum \log(p)$   \\ \hline \hline
BMA             & -2.16              & -162.11             & Average        & -2.00           & -150.07               \\ \hline
\multicolumn{3}{c||}{\textbf{Individual models}}           & \multicolumn{3}{c}{\textbf{Best N-average, $rw=20$}}\\ \hline
Best            & -2.08              & -156.04             & N=1            & -2.09           & -156.84               \\
Median          & -2.24              & -168.08             & N=2            & -2.06           & -154.79               \\ \cline{1-3}
\multicolumn{3}{c||}{\textbf{Dynamic Model Averaging}}     & N=3            & -1.99           & -149.57               \\ \cline{1-3}
$\alpha=  0.95$ & -2.02              & -151.35             & N=4            & -2.01           & -151.03               \\ 
$\alpha=  0.90$ & -1.97              & -147.58             & N=5            & -1.99           & -149.46               \\
$\alpha=  0.80$ & -1.91              & -143.60             & N=6            & -1.99           & -148.85               \\ 
$\alpha=  0.70$ & -1.90              & -142.40             & N=7            & -1.96           & -147.16               \\ \hline
\multicolumn{3}{c||}{$\mbox{LDF}_{\mbox{s}, \mbox{a}}^2$}  & \multicolumn{3}{c}{$\mbox{LDF}_{\mbox{s}, \mbox{s}}^2$}  \\ \hline           
$\alpha =1.00$  & -1.94              & -145.60             &$\alpha =1.00$  & -1.92           & -144.00               \\
$\alpha =0.95$  & -1.94              & -145.11             &$\alpha =0.95$  & -1.92           & -144.34               \\
$\alpha =0.90$  & -1.89              & -141.85             &$\alpha =0.90$  & -1.93           & -144.44               \\
$\alpha =0.80$  & -1.89              & -141.76             &$\alpha =0.80$  & -1.93           & -144.42               \\
$\alpha =0.70$  & -1.88              & -141.22             &$\alpha =0.70$  & -1.92           & -144.28                               
\end{tabular}%

==> tables/table_ecb_short.tex <==
\begin{tabular}{c|c|c||c|c|c}
\textbf{Model}  & $\bar{\log(p)}$    & $\sum \log(p)$      & \textbf{Model} & $\bar{\log(p)}$ & $\sum \log(p)$   \\ \hline \hline
BMA             & -2.16              & -162.11             & Average        & -2.00           & -150.07               \\ \hline
\multicolumn{6}{c}{\textbf{Individual models}}           \\ \hline
Best & -2.08 & -156.04 & Median & -2.24 & -168.08\\ \hline
\multicolumn{6}{c}{\textbf{Best N-average, $rw=20$}}\\ \hline
    N=1            & -2.09           & -156.84 &   N=5            & -1.99           & -149.46                  \\
 N=2            & -2.06           & -154.79   & N=6            & -1.99           & -148.85                \\ 
    N=3            & -1.99           & -149.57   &  N=7            & -1.96           & -147.16             \\ 
      N=4            & -2.01           & -151.03  
     &              &              &           \\ 
\end{tabular}%

==> tables/table_fx_short.tex <==
\begin{tabular}{c|c|c||c|c|c||c|c|c||c|c|c}
\multicolumn{6}{c||}{Large model pool} & \multicolumn{6}{c}{Small model pool}\\ \hline \hline
\multicolumn{3}{c||}{Model Averaging}   & \multicolumn{3}{c||}{Model Selection} & \multicolumn{3}{c||}{Model Averaging}   & \multicolumn{3}{c}{Model Selection} \\ \hline 
\textbf{Model} & \textbf{$\bar{\log(p)}$} & \textbf{$\sum \log(p)$}       & \textbf{Model}               & \textbf{$\bar{\log(p)}$}        & \textbf{$\sum \log(p)$}  & \textbf{Model} & \textbf{$\bar{\log(p)}$} & \textbf{$\sum \log(p)$}       & \textbf{Model}               & \textbf{$E[log(p)]$}        & \textbf{$\sum log(p)$}   \\ \hline \hline
Average         & 20.82      & 5037.57             & RW                            & 21.77               & 5267.81         & BPS           & 21.60 & 5227.56 & Average      & 21.71 & 5253.55   \\
BMA             & 21.91      & 5302.83             & Best                          & 21.78               & 5271.02         & Best-4 avg.   & 22.10 & 5349.11 & Best         & 21.77 & 5267.81     \\
\end{tabular}%

==> tables/table_simulation_short.tex <==
\begin{tabular}{c|c|c|c|c||c|c|c|c|c}
\textbf{Model}    & $\bar{\bar{\log(p)}}$   & $\sigma[\bar{log(p)}]$ & $\overline{\sum log(p)}$ &$\sigma[\sum log(p)]$& \textbf{Model}  & $\bar{\bar{\log(p)}}$   & $\sigma[\bar{log(p)}]$ & $\overline{\sum log(p)}$ &$\sigma[\sum log(p)]$  \\
\hline
\hline
BMA               & -4.34           & 0.05               & -8601.11	      & 107.41	        & BPS               & -0.73           &$\text{N/A}^*$& -1444.08 &$\text{N/A}^*$\\
\hline 
\multicolumn{10}{c}{\textbf{Best N-average, rolling-window=5}}  \\
\hline
N=1               & -0.71           & 0.02               & -1404.45        & 45.73           &  N=4               & -0.52           & 0.02               & -1033.21        & 33.46        \\
N=2               & -0.55           & 0.03               & -1080.86	       & 52.25	         & N=5               & -0.54           & 0.02               & -1063.02        & 31.84	      \\
N=3               & -0.52           & 0.03               & -1031.68	       & 49.74           & N=6               & -0.57           & 0.01               & -1134.41	       & 27.37          \\
\end{tabular}%

==> tables/table_usinf_short.tex <==
\begin{tabular}{c|c|c||c|c|c}
\textbf{Model}    & $\bar{\log(p)}$   & $\sum \log(p)$ & \textbf{Model}  & $\bar{\log(p)}$& $\sum \log(p)$  \\
\hline
\hline
BMA               & -0.03           & -2.97	        & BPS               & 0.06           & 6.10 \\
\hline 
\multicolumn{3}{c||}{\textbf{Best N-average, $rw=20$}} & \multicolumn{3}{c}{\textbf{Single models}}  \\
\hline
N=1               & -0.06           & -5.75        & $M_1$            & -0.08           & -7.77      \\
N=2               & -0.01           & -0.87	       & $M_2$            & -0.02           & -2.48      \\
N=3               & -0.01           & -1.40        & $M_3$            & -0.03           & -2.97      \\
N=4               & -0.03           & -3.03        & $M_4$            & -0.17           & -16.65                           
\end{tabular}%
